EdgeDiT: Hardware-Aware Diffusion Transformers for Efficient On-Device Image Generation

Diffusion Transformers (DiT) have established a new state-of-the-art in high-fidelity image synthesis; however, their massive computational complexity and memory requirements hinder local deployment on resource-constrained edge devices. In this paper, we introduce EdgeDiT, a family of hardware-efficient generative transformers specifically engineered for mobile Neural Processing Units (NPUs), such as the Qualcomm Hexagon and Apple Neural Engine (ANE). By leveraging a hardware-aware optimization framework, we systematically identify and prune structural redundancies within the DiT backbone that are particularly taxing for mobile data-flows. Our approach yields a series of lightweight models that achieve a 20-30% reduction in parameters, a 36-46% decrease in FLOPs, and a 1.65-fold reduction in on-device latency without sacrificing the scaling advantages or the expressive capacity of the original transformer architecture. Extensive benchmarking demonstrates that EdgeDiT offers a superior Pareto-optimal trade-off between Frechet Inception Distance (FID) and inference latency compared to both optimized mobile U-Nets and vanilla DiT variants. By enabling responsive, private, and offline generative AI directly on-device, EdgeDiT provides a scalable blueprint for transitioning large-scale foundation models from high-end GPUs to the palm of the user.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/3_methodology_trash.tex <==
\section{Method}

Our goal is to design edge-efficient variants of Diffusion Transformers derived from the DiT-XL/2 \cite{peebles2023dit} baseline that preserve generative performance while reducing computational and memory overhead for edge deployment.

Importantly, theoretical compute metrics such as FLOPs or GMACs do not always accurately predict practical latency on mobile Neural Processing Units (NPUs). These accelerators are highly optimized for specific operations such as matrix multiplications (GEMM). As a result, reducing arithmetic operations alone does not necessarily guarantee proportional improvements in edge latency.

To address this gap, we propose a hardware-aware architecture exploration framework. We construct a structured search space of lightweight surrogate transformer blocks aligned with edge hardware constraints. These surrogates are trained using feature-wise knowledge distillation and then assembled to form candidate architectures. The resulting candidates are evaluated using multi-objective Bayesian optimization to discover Pareto-optimal models in the hardware–performance trade-off space. The most balanced architecture from this frontier is selected as our final model, \textbf{EdgeDiT}. An overview of the proposed framework is illustrated in Fig.~X.

\subsection{Overview of EdgeDiT}

EdgeDiT is designed using a hardware-aware methodology that targets efficient execution on mobile NPUs such as Qualcomm Hexagon and Apple Neural Engine. Starting from the DiT-XL/2 architecture, we decompose the network into modular transformer blocks and construct surrogate variants that are more suitable for edge deployment.

These surrogate components are trained independently through feature-wise knowledge distillation. Candidate architectures are then assembled by combining different surrogate blocks, and the resulting design space is explored using multi-objective Bayesian optimization. This pipeline enables efficient discovery of architectures that achieve strong generative performance while minimizing hardware latency.

\subsection{Hardware Decomposition of Diffusion Transformers}

Diffusion Transformers (DiT) \cite{peebles2023dit} operate on latent image representations by treating them as sequences of tokens processed by transformer blocks. Given an input image $x$, it is first encoded into a latent representation using a variational autoencoder. The latent representation is then divided into non-overlapping patches of size $p \times p$, producing a sequence of tokens that form the input to the transformer backbone.

A DiT model consists of a stack of $L$ transformer blocks ($L = 28$ for DiT-XL/2). Each block contains two primary components:

\begin{itemize}
\item Multi-head self-attention (MHSA)
\item Feed-forward network (FFN) with expansion ratio $r$
\end{itemize}

Formally, a transformer block can be expressed as

\begin{equation}
h_{l+1} = h_l + MHSA(LN(h_l)) + FFN(LN(h_l)),
\end{equation}

where $h_l$ denotes the hidden representation at layer $l$ and $LN$ denotes layer normalization.

Although DiT models provide strong generative performance, their large number of layers and high-dimensional hidden representations introduce significant computational and memory overhead. To address this challenge, we decompose the DiT architecture into smaller hardware-friendly building blocks and construct a structured architecture search space.

\subsection{Hardware-Aware Architecture Design}

Our hardware-aware search space consists of surrogate transformer blocks designed to reduce computation and memory footprint while preserving the representational capacity of the original model.

Specifically, we consider three types of architectural modifications:

\begin{enumerate}
\item \textbf{Block removal}: Every two consecutive DiT layers can be replaced with a single layer, effectively reducing network depth.
\item \textbf{MLP ratio modification}: The expansion ratio of the FFN block in DiT layers is varied, with expansion factor
\[
r \in \{2, 4\},
\]
which reduces both parameter count and FLOPs.
\item \textbf{Hidden dimension reduction}: The internal projection dimension of transformer blocks is reduced to lower-rank representations,
\[
d \in \{512,1152\}.
\]
\end{enumerate}

These surrogates are constructed in two stages:

\textbf{Stage 1: Block removal.}

Each pair of two consecutive DiT layers is replaced by a single surrogate layer. This results in a search space of

\[
2 \times 2 \times  ....  \text{(14 times)} \times 2 = 2^{14}
\]

possible configurations.

\textbf{Stage 2: Structural simplification.}

For each layer, we choose between modified MLP ratios or reduced hidden dimensions. This introduces six possible configurations per layer, producing a search space of
\[
4 \times 4 \times ...  \text{(28 times)} \times 4 = 4^{28}
\]

Together, these design choices form a large hardware-aware architecture space. Figure \ref{fig:surr} illustrates the complete surrogate search space design.

\begin{figure*}
    \centering
    \includegraphics[width=1.0\linewidth]{sec/figures/surr.png}
    % \caption{Surrogates design}
    \caption{hardware-aware surrogates search space design}
    \label{fig:surr}
\end{figure*}

\subsection{Feature-wise Knowledge Distillation}

Training every candidate architecture in the search space from scratch would be computationally infeasible. To address this challenge, we adopt a feature-wise knowledge distillation strategy.

In this approach, each surrogate block learns to mimic the behavior of the corresponding block in the teacher network. Let $T_l(x)$ denote the output feature of the $l$-th block in the teacher model and $S_l(x)$ denote the output of the surrogate block for input features $x$. The distillation loss is defined as

\begin{equation}
L_{KD}^{l} = \|T_l(x) - S_l(x)\|_2^2.
\end{equation}

Surrogate training is performed in two stages corresponding to the architecture decomposition:

\textbf{Stage 1: Block removal.}

Each pair of consecutive DiT layers acts as the teacher model, and their behavior is distilled into a single student transformer layer.

\textbf{Stage 2: Structural simplification.}

In the second stage, the original DiT layer serves as the teacher while the modified layers with different MLP ratios or reduced hidden dimensions act as students.

Because all surrogate blocks are distilled independently, this training process is massively parallel and computationally lightweight. In total, we obtain 14 surrogate blocks in Stage 1 and $5 \times 28 = 140$ surrogate blocks in Stage 2.

This progressive training strategy preserves the local behavior of the DiT-XL/2 architecture while enabling efficient construction of lightweight candidate networks.

\subsection{Assembling Candidate Architectures}

Once surrogate blocks are trained, candidate diffusion transformer architectures are constructed by combining different configurations of these components.

Each candidate architecture is represented by a configuration vector

\begin{equation}
a = (b_1, b_2, \dots, b_L),
\end{equation}

where $b_i$ denotes the block type selected for layer $i$. The block type may correspond to the original DiT block or one of the surrogate variants.

Given configuration $a$, the network is assembled by selecting the corresponding surrogate block for each layer. Because surrogate blocks are pre-trained through distillation, candidate architectures can be evaluated efficiently without exhaustive retraining.

\subsection{Optimization in Hardware-Aligned Space}

To identify efficient architectures within the search space, we formulate model selection as a multi-objective optimization problem.

Let $f(a)$ denote a performance metric such as Fréchet Inception Distance (FID) and $g(a)$ denote a hardware cost metric such as peak memory usage or edge latency. Our objective is to find architectures that satisfy

\begin{equation}
\max_{a \in A} f(a), \quad \min_{a \in A} g(a).
\end{equation}

To explore the architecture space efficiently, we employ multi-objective Bayesian optimization (MOBO). A Gaussian process model predicts objective values for candidate architectures based on previously evaluated configurations. New architectures are then selected using an acquisition function that balances exploration and exploitation.

In practice, we evaluate candidate architectures by generating a set of images and computing their FID score while measuring edge latency on the target hardware. This allows us to identify Pareto-optimal architectures that provide the best trade-offs between generative quality and hardware efficiency.

\subsection{Computational Complexity Analysis}

We further analyze the computational complexity of EdgeDiT relative to the original DiT architecture. In transformer models, the dominant computational cost arises from the self-attention mechanism. For a sequence length $N$ and hidden dimension $d$, the complexity of a self-attention layer is

\begin{equation}
\mathcal{O}(N^2 d).
\end{equation}

By reducing network depth, lowering hidden dimensions, and adjusting MLP expansion ratios, EdgeDiT significantly decreases both parameter count and FLOPs compared to the baseline DiT architecture. These architectural changes also reduce memory bandwidth requirements, which is a critical factor for efficient execution on mobile NPUs.

As a result, EdgeDiT achieves substantial improvements in inference latency while maintaining competitive generative performance.

==> sec/Sravanth_Gen/Introduction.tex <==
\section{Introduction}

Diffusion models have recently emerged as a dominant paradigm for high-fidelity image generation. Early approaches such as Denoising Diffusion Probabilistic Models (DDPM) \cite{ho2020ddpm} and Denoising Diffusion Implicit Models (DDIM) \cite{song2021ddim} demonstrated that iterative denoising processes can generate high-quality images by gradually transforming Gaussian noise into structured samples. These models were initially built upon convolutional U-Net backbones, which became the de facto architecture for diffusion-based image synthesis.

Recent advances have shifted toward transformer-based generative architectures. Diffusion Transformers (DiT) \cite{peebles2023dit} replace convolutional U-Nets with Vision Transformer backbones, enabling improved scalability and better utilization of large-scale training data. Building on this paradigm, several works have explored architectural improvements and training strategies for transformer-based diffusion models. Masked Diffusion Transformer (MDT) \cite{gao2023mdt} introduced masked modeling objectives that significantly improve synthesis quality. Scalable Interpolant Transformers (SiT) \cite{siT2024} further unified diffusion and flow-based generative modeling under a transformer-based framework. More recently, representation alignment techniques \cite{li2024representation} have demonstrated that training diffusion transformers can be simplified and stabilized through improved feature alignment strategies.

Parallel efforts have also investigated alternative backbones for diffusion models. For instance, state-space models have recently been explored as efficient sequence modeling alternatives to transformers, leading to architectures such as diffusion models with state-space backbones \cite{statespace2024diffusion}. These approaches aim to improve scalability and computational efficiency while preserving generative quality.

Despite these advances, the deployment of diffusion transformers on edge devices remains challenging. State-of-the-art DiT architectures require substantial computational resources, large memory footprints, and high inference latency, making them impractical for mobile and embedded platforms. While cloud-based inference mitigates these limitations, it introduces privacy concerns, network dependency, and increased energy consumption.

In this work, we address the challenge of bringing transformer-based diffusion models to resource-constrained hardware. We introduce \textbf{NanoDiT}, a family of lightweight diffusion transformers specifically optimized for mobile Neural Processing Units (NPUs) such as Qualcomm Hexagon and Apple Neural Engine (ANE). Our approach applies hardware-aware architectural optimization to identify and eliminate redundant structures within the DiT backbone, reducing both parameter count and computational complexity while preserving generative capacity.

Through systematic model redesign and pruning strategies, NanoDiT achieves a 20--30\% reduction in parameters and a 25--40\% decrease in FLOPs compared to baseline DiT architectures. Extensive experiments demonstrate that NanoDiT achieves competitive Fréchet Inception Distance (FID) while significantly reducing inference latency on edge hardware.

Our contributions are summarized as follows:

\begin{itemize}
\item We propose NanoDiT, a hardware-aware diffusion transformer architecture designed for efficient on-device generation.
\item We introduce structural simplifications and pruning strategies tailored for mobile NPUs.
\item We demonstrate improved Pareto trade-offs between generation quality and inference efficiency compared to existing DiT variants.
\item We provide empirical evidence that transformer-based diffusion models can be effectively scaled down for real-world edge deployment.
\end{itemize}

==> sec/Sravanth_Gen/Limitations.tex <==
\section{Limitations and Future Work}

While EdgeDiT demonstrates promising results for enabling diffusion transformers on mobile hardware, several limitations remain.

First, our experiments are conducted primarily using the DiT-XL/2 architecture as the base teacher model. Although the proposed surrogate-based architecture search framework is model-agnostic in principle, we did not extend the search to other transformer-based diffusion families such as SiT or MDT due to computational constraints. Exploring the effectiveness of our framework across multiple generative transformer backbones remains an important direction for future work.

Second, the goal of this work is not to design the most parameter-efficient diffusion model, but rather to propose a general hardware-aware optimization framework that can automatically discover efficient architectures within a given model family. Recent architectures such as SiT and other emerging transformer variants may offer stronger baseline performance at comparable model scales. Integrating our surrogate-based search and hardware-aware optimization pipeline with these newer model families could further improve efficiency-performance trade-offs.

Third, while we evaluate hardware performance on representative mobile NPUs including Qualcomm Hexagon and Apple Neural Engine (ANE), the hardware-aware search space could be further specialized for different accelerator architectures. Future work may explore device-specific search spaces that adapt architectural decisions to diverse hardware backends such as GPUs, NPUs, and emerging AI accelerators.

Finally, our current implementation trains only a subset of candidate architectures end-to-end due to the high computational cost of diffusion model training. Scaling the search process with larger compute budgets could enable training a broader set of candidate models and potentially discovering even more efficient architectures.

Overall, we believe that the proposed hardware-aware surrogate search framework provides a flexible foundation for designing efficient generative transformers and can be extended to future diffusion architectures and edge AI systems.


==> sec/Sravanth_Gen/Method.tex <==
\section{Method}

Our goal is to design edge-efficient variants of Diffusion Transformers derived from the DiT-XL/2 \cite{peebles2023dit} baseline that preserve generative performance while reducing computational and memory overhead for edge deployment.

Importantly, theoretical compute metrics such as FLOPs or GMACs do not always accurately predict practical latency on mobile Neural Processing Units (NPUs). These accelerators are highly optimized for specific operations such as matrix multiplications (GEMM). As a result, reducing arithmetic operations alone does not necessarily guarantee proportional improvements in edge latency.

To address this gap, we propose a hardware-aware architecture exploration framework. We construct a structured search space of lightweight surrogate transformer blocks aligned with edge hardware constraints. These surrogates are trained using feature-wise knowledge distillation and then assembled to form candidate architectures. The resulting candidates are evaluated using multi-objective Bayesian optimization to discover Pareto-optimal models in the hardware–performance trade-off space. The most balanced architecture from this frontier is selected as our final model, \textbf{NanoDiT}. An overview of the proposed framework is illustrated in Fig.~X.

\subsection{Overview of NanoDiT}

NanoDiT is designed using a hardware-aware methodology that targets efficient execution on mobile NPUs such as Qualcomm Hexagon and Apple Neural Engine. Starting from the DiT-XL/2 architecture, we decompose the network into modular transformer blocks and construct surrogate variants that are more suitable for edge deployment.

These surrogate components are trained independently through feature-wise knowledge distillation. Candidate architectures are then assembled by combining different surrogate blocks, and the resulting design space is explored using multi-objective Bayesian optimization. This pipeline enables efficient discovery of architectures that achieve strong generative performance while minimizing hardware latency.

\subsection{Hardware Decomposition of Diffusion Transformers}

Diffusion Transformers (DiT) \cite{peebles2023dit} operate on latent image representations by treating them as sequences of tokens processed by transformer blocks. Given an input image $x$, it is first encoded into a latent representation using a variational autoencoder. The latent representation is then divided into non-overlapping patches of size $p \times p$, producing a sequence of tokens that form the input to the transformer backbone.

A DiT model consists of a stack of $L$ transformer blocks ($L = 28$ for DiT-XL/2). Each block contains two primary components:

\begin{itemize}
\item Multi-head self-attention (MHSA)
\item Feed-forward network (FFN) with expansion ratio $r$
\end{itemize}

Formally, a transformer block can be expressed as

\begin{equation}
h_{l+1} = h_l + MHSA(LN(h_l)) + FFN(LN(h_l)),
\end{equation}

where $h_l$ denotes the hidden representation at layer $l$ and $LN$ denotes layer normalization.

Although DiT models provide strong generative performance, their large number of layers and high-dimensional hidden representations introduce significant computational and memory overhead. To address this challenge, we decompose the DiT architecture into smaller hardware-friendly building blocks and construct a structured architecture search space.

\subsection{Hardware-Aware Architecture Design}

Our hardware-aware search space consists of surrogate transformer blocks designed to reduce computation and memory footprint while preserving the representational capacity of the original model.

Specifically, we consider three types of architectural modifications:

\begin{enumerate}
\item \textbf{Block removal}: Every two consecutive DiT layers can be replaced with a single layer, effectively reducing network depth.
\item \textbf{MLP ratio modification}: The expansion ratio of the FFN block in DiT layers is varied, with expansion factor
\[
r \in \{1,2,3,4\},
\]
which reduces both parameter count and FLOPs.
\item \textbf{Hidden dimension reduction}: The internal projection dimension of transformer blocks is reduced to lower-rank representations,
\[
d \in \{512,1152\}.
\]
\end{enumerate}

These surrogates are constructed in two stages:

\textbf{Stage 1: Block removal.}

Each pair of two consecutive DiT layers is replaced by a single surrogate layer. This results in a search space of

\[
2^{14}
\]

possible configurations.

\textbf{Stage 2: Structural simplification.}

For each layer, we choose between modified MLP ratios or reduced hidden dimensions. This introduces six possible configurations per layer, producing a search space of

\[
6^{28}.
\]

Together, these design choices form a large hardware-aware architecture space. Figure~1 illustrates the complete surrogate search space design.

\subsection{Feature-wise Knowledge Distillation}

Training every candidate architecture in the search space from scratch would be computationally infeasible. To address this challenge, we adopt a feature-wise knowledge distillation strategy.

In this approach, each surrogate block learns to mimic the behavior of the corresponding block in the teacher network. Let $T_l(x)$ denote the output feature of the $l$-th block in the teacher model and $S_l(x)$ denote the output of the surrogate block for input features $x$. The distillation loss is defined as

\begin{equation}
L_{KD}^{l} = \|T_l(x) - S_l(x)\|_2^2.
\end{equation}

Surrogate training is performed in two stages corresponding to the architecture decomposition:

\textbf{Stage 1: Block removal.}

Each pair of consecutive DiT layers acts as the teacher model, and their behavior is distilled into a single student transformer layer.

\textbf{Stage 2: Structural simplification.}

In the second stage, the original DiT layer serves as the teacher while the modified layers with different MLP ratios or reduced hidden dimensions act as students.

Because all surrogate blocks are distilled independently, this training process is massively parallel and computationally lightweight. In total, we obtain 14 surrogate blocks in Stage 1 and $5 \times 28 = 140$ surrogate blocks in Stage 2.

This progressive training strategy preserves the local behavior of the DiT-XL/2 architecture while enabling efficient construction of lightweight candidate networks.

\subsection{Assembling Candidate Architectures}

Once surrogate blocks are trained, candidate diffusion transformer architectures are constructed by combining different configurations of these components.

Each candidate architecture is represented by a configuration vector

\begin{equation}
a = (b_1, b_2, \dots, b_L),
\end{equation}

where $b_i$ denotes the block type selected for layer $i$. The block type may correspond to the original DiT block or one of the surrogate variants.

Given configuration $a$, the network is assembled by selecting the corresponding surrogate block for each layer. Because surrogate blocks are pre-trained through distillation, candidate architectures can be evaluated efficiently without exhaustive retraining.

\subsection{Optimization in Hardware-Aligned Space}

To identify efficient architectures within the search space, we formulate model selection as a multi-objective optimization problem.

Let $f(a)$ denote a performance metric such as Fréchet Inception Distance (FID) and $g(a)$ denote a hardware cost metric such as peak memory usage or edge latency. Our objective is to find architectures that satisfy

\begin{equation}
\max_{a \in A} f(a), \quad \min_{a \in A} g(a).
\end{equation}

To explore the architecture space efficiently, we employ multi-objective Bayesian optimization (MOBO). A Gaussian process model predicts objective values for candidate architectures based on previously evaluated configurations. New architectures are then selected using an acquisition function that balances exploration and exploitation.

In practice, we evaluate candidate architectures by generating a set of images and computing their FID score while measuring edge latency on the target hardware. This allows us to identify Pareto-optimal architectures that provide the best trade-offs between generative quality and hardware efficiency.

\subsection{Computational Complexity Analysis}

We further analyze the computational complexity of NanoDiT relative to the original DiT architecture. In transformer models, the dominant computational cost arises from the self-attention mechanism. For a sequence length $N$ and hidden dimension $d$, the complexity of a self-attention layer is

\begin{equation}
\mathcal{O}(N^2 d).
\end{equation}

By reducing network depth, lowering hidden dimensions, and adjusting MLP expansion ratios, NanoDiT significantly decreases both parameter count and FLOPs compared to the baseline DiT architecture. These architectural changes also reduce memory bandwidth requirements, which is a critical factor for efficient execution on mobile NPUs.

As a result, NanoDiT achieves substantial improvements in inference latency while maintaining competitive generative performance.

==> sec/Sravanth_Gen/Related_works.tex <==
\section{Related Work}

\subsection{Diffusion Models}

Diffusion models have achieved remarkable success in generative modeling across a variety of visual tasks. Denoising Diffusion Probabilistic Models (DDPM)~\cite{ho2020ddpm} introduced a probabilistic formulation for image generation based on iterative denoising of Gaussian noise. Subsequent improvements such as Improved DDPM~\cite{nichol2021improved} enhanced sampling efficiency and training stability. Latent Diffusion Models (LDM)~\cite{rombach2022ldm} further improved scalability by performing diffusion in a compressed latent space, significantly reducing computational requirements while maintaining high visual fidelity.

\subsection{Diffusion Transformers}

Transformer architectures have recently been adopted as powerful backbones for diffusion models. Diffusion Transformers (DiT)~\cite{peebles2023dit} replace convolutional U-Net architectures with transformer blocks operating on latent tokens, demonstrating strong scaling properties for generative modeling. Several works have further explored architectural improvements to diffusion transformers. Masked Diffusion Transformer (MDT) and its improved variant MDTv2~\cite{gao2023mdtv2} introduce masked latent modeling strategies that improve contextual reasoning and accelerate training. 

Scalable Interpolant Transformers (SiT)~\cite{ma2024sit} extend diffusion transformers to a broader generative modeling framework that unifies diffusion and flow-based models through stochastic interpolants, enabling flexible training objectives and improved performance across model scales. 1

Other recent works investigate alternative architectural backbones for diffusion models. For instance, state-space model based diffusion architectures replace attention mechanisms with structured state-space layers to improve scalability and reduce computational complexity. These approaches highlight ongoing efforts to improve both the scalability and efficiency of transformer-based diffusion models.

\subsection{Efficient and Lightweight Diffusion Models}

The growing computational cost of diffusion models has motivated research into lightweight diffusion architectures. MobileDiffusion~\cite{mobilediffusion} proposes architectural simplifications designed for mobile hardware to enable efficient on-device diffusion inference. Other works explore structured pruning and token sparsification techniques to reduce redundancy in diffusion transformers. 

Additionally, efficient training strategies have been explored to reduce the cost of training large diffusion models. For example, masked training strategies and representation alignment approaches have been shown to significantly simplify the training process of diffusion transformers while maintaining strong generative performance~\cite{representation_alignment}.

\subsection{Model Compression and Architecture Search}

Model compression techniques such as pruning, knowledge distillation, and neural architecture search have been widely used to obtain compact neural networks suitable for deployment on edge hardware. Knowledge distillation~\cite{hinton2015distilling} allows smaller student networks to mimic the behavior of larger teacher models while preserving performance. Automated architecture search methods such as Bayesian optimization~\cite{snoek2012practical} enable systematic exploration of large architecture spaces under hardware constraints.

In contrast to prior work that primarily focuses on manual architecture design or pruning strategies, our work introduces a surrogate-based architecture search framework that combines feature-wise knowledge distillation and multi-objective Bayesian optimization to discover efficient diffusion transformer architectures optimized for edge deployment.

